Multi-task Retrieval for Knowledge-Intensive Tasks

Retrieving relevant contexts from a large corpus is a crucial step for tasks such as open-domain question answering and fact checking. Although neural retrieval outperforms traditional methods like tf-idf and BM25, its performance degrades considerably when applied to out-of-domain data. Driven by the question of whether a neural retrieval model can be universal and perform robustly on a wide variety of problems, we propose a multi-task trained model. Our approach not only outperforms previous methods in the few-shot setting, but also rivals specialised neural retrievers, even when in-domain training data is abundant. With the help of our retriever, we improve existing models for downstream tasks and closely match or improve the state of the art on multiple benchmarks.

==> tables/dev_KILT_scores.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{   
\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l@{\hskip 2em}rrrrrrrrrrr}
 \toprule
    \multicolumn{2}{r}{Fact Check.}  & \multicolumn{3}{c}{Entity Linking} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
model & \textbf{FEV}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{WoW}   \\
\midrule
 & \multicolumn{6}{c|}{KILT-AC} & \multicolumn{3}{c|}{KILT-EM} & \multicolumn{1}{c|}{-RL} & \multicolumn{1}{c}{-F1} \\
\midrule
BART + DPR & 48.25 & - & - & - & 11.56 & 29.08 & 31.62 & 1.96 & 32.56 & 2.87 & 0.0 \\
BART + Multi-task DPR & 66.99 & 82.77 & - & - & - & 49.73 & 35.0 & 9.2 & 42.58 & - & 7.4 \\
BART + Multi-task DPR v2 & 65.49 & 83.98 & - & - & - & 50.45 & 33.09 & 11.41 & 40.92 & - & 7.04 \\
 \bottomrule
\end{tabular}
}
\caption{Dev KILT scores. }
\label{tab:KILT_table}
\end{table*}


==> tables/dev_downstream.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{   
\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l@{\hskip 2em}rrrrrrrrrrr}
 \toprule
    \multicolumn{2}{r}{Fact Check.}  & \multicolumn{3}{c}{Entity Linking} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
  model & \textbf{FEV}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{WoW}   \\
\midrule
 & \multicolumn{6}{c|}{Accuracy} & \multicolumn{3}{c|}{Exact Match} & \multicolumn{1}{c|}{RL} & \multicolumn{1}{c}{F1} \\
\midrule
BART + DPR & 88.11 & - & - & - & 56.7 & 34.96 & 45.05 & 25.75 & 59.28 & 18.53 & 15.03 \\
BART + Multi-task DPR & 88.54 & 82.77 & - & - & - & 56.98 & 45.08 & 32.52 & 59.74 & - & 14.89 \\
BART + Multi-task DPR v2 & 87.96 & 83.98 & - & - & - & 58.08 & 41.83 & 32.83 & 57.01 & - & 15.29 \\
 \bottomrule
\end{tabular}
}
\caption{Dev downstream performance.}
\label{tab:downstream_table}
\end{table*}


==> tables/old_retrieval_page.tex <==
\begin{table*}[t]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l@{\hskip 3em}rrrrrrrrrrr}
 \toprule
   \multicolumn{2}{r}{Fact Check.}  & \multicolumn{3}{c}{Entity Linking} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
 model  & \textbf{FEV}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{WoW}   \\
\midrule
All-KILT & \textbf{74.72} & \textbf{83.78} & --- & --- & \textbf{69.18} & \underline{77.23} & \underline{61.51} & \underline{44.21} & \underline{61.95} & --- & 39.70 \\
FEVER & 45.08 & 5.62 & --- & --- & 19.50 & 42.88 & 36.69 & 23.18 & 45.08 & --- & \textbf{41.27} \\
AY2 & 47.36 & \underline{81.77} & --- & --- & 5.52 & 8.94 & 10.22 & 11.69 & 15.11 & --- & 17.59 \\
T-REx & 45.63 & 1.05 & --- & --- & \underline{69.08} & 71.64 & 17.10 & 22.31 & 18.10 & --- & 4.02 \\
zsRE & \underline{70.10} & 0.42 & --- & --- & 68.34 & \textbf{97.74} & 25.98 & 22.23 & 28.68 & --- & 10.40 \\
NQ & 68.16 & 1.44 & --- & --- & 31.78 & 61.12 & \textbf{63.24} & 29.39 & 48.39 & --- & 30.77 \\
HoPo & 56.18 & 2.07 & --- & --- & 35.76 & 44.44 & 35.60 & \textbf{46.63} & 41.18 & --- & 23.51 \\
TQA & 70.06 & 4.95 & --- & --- & 32.22 & 60.37 & 45.01 & 32.62 & \textbf{65.12} & --- & \underline{41.17} \\
\bottomrule
\end{tabular}
}
\caption{Page-level R-Precision on KILT validation data.}
\label{tab:page-retrieval-dev}
\end{table*}

==> tables/old_retrieval_para.tex <==
\begin{table*}[t]
\centering

\begin{tabular}{l@{\hskip 3em}rrrrrrr}
 \toprule
   & \multicolumn{1}{r}{Fact Check.}  & \multicolumn{2}{c}{Slot Filling} & \multicolumn{3}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
 model  & \textbf{FEV}  & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{WoW}   \\
\midrule
Shared & \textbf{46.96} & 53.54 & \underline{41.70} & \textbf{28.80} & \underline{38.42} & \underline{24.56} & \textbf{24.07} \\
BM25 & 40.06 & 51.64 & 52.98 & 14.20 & 38.38 & 16.16 & 18.41 \\
\midrule
\multicolumn{8}{c}{Task-specific models}\\
\midrule
FEVER & \underline{43.92} & 10.02 & 19.98 & 18.05 & 17.59 & 22.24 & 19.85\\
AY2 & & 4.08 & & 6.77 & 10.71 & 8.47 & 13.08 \\
T-REx & 25.22 & \textbf{58.54} & 40.95 & 8.71 & 15.63 & 8.06 & 1.83 \\
zsRE & & \underline{57.40} & \textbf{78.81} & 13.81 & 18.35 & 14.44 & 2.09 \\
NQ & 14.81 & 7.20 & 12.92 & \underline{28.13} & 11.33 & 14.42 & 11.81 \\
HoPo & 40.03 & 27.62 & 31.15 & 23.26 & \textbf{43.47} & \textbf{29.37} & 16.02 \\
TQA & 10.68 & 12.52 & 17.43 & 12.97 & 13.05 & 23.79 & 8.11 \\
WoW & 42.79 & 18.52 & 35.26 & 22.52 & 17.66 & 23.15 & \underline{20.73} \\
\bottomrule
\end{tabular}

\caption{Passage-level $R$-precision on KILT validation data.}
\label{tab:leave-one-out}
\end{table*}

==> tables/test_KILT_scores.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{   
\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l@{\hskip 2em}rrrrrrrrrrr}
 \toprule
    \multicolumn{2}{r}{Fact Check.}  & \multicolumn{3}{c}{Entity Linking} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
model & \textbf{FEV}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{WoW}   \\
\midrule
 & \multicolumn{6}{c|}{KILT-AC} & \multicolumn{3}{c|}{KILT-EM} & \multicolumn{1}{c|}{-RL} & \multicolumn{1}{c}{-F1} \\
\midrule
BART + DPR & 47.68 & 75.49 & 45.2 & 46.87 & 11.12 & 18.91 & 30.06 & 1.96 & 31.4 & \textbf{1.9} & 4.52 \\
BART + Multi-task DPR & 63.94 & 82.61 & - & - & - & 50.64 & 29.09 & 9.53 & 42.36 & - & 7.25 \\
 \bottomrule
\end{tabular}
}
\caption{Test KILT scores. }
\label{tab:KILT_table}
\end{table*}


==> tables/test_downstream.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{   
\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{l@{\hskip 2em}rrrrrrrrrrr}
 \toprule
    \multicolumn{2}{r}{Fact Check.}  & \multicolumn{3}{c}{Entity Linking} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
  model & \textbf{FEV}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{WoW}   \\
\midrule
 & \multicolumn{6}{c|}{Accuracy} & \multicolumn{3}{c|}{Exact Match} & \multicolumn{1}{c|}{RL} & \multicolumn{1}{c}{F1} \\
\midrule
BART + DPR & 86.74 & 75.49 & 45.2 & 46.87 & 59.16 & 30.43 & 41.27 & 25.18 & 58.55 & 17.41 & 15.55 \\
BART + Multi-task DPR & 86.32 & 82.61 & - & -  & - & 57.95 & 39.75 & 31.77 & 59.60 & - & 15.33 \\
 \bottomrule
\end{tabular}
}
\caption{Test downstream performance.}
\label{tab:downstream_table}
\end{table*}

